The TESS-Keck Survey. XVI. Mass Measurements for 12 Planets in Eight Systems

With JWST's successful deployment and unexpectedly high fuel reserves, measuring the masses of sub-Neptunes transiting bright, nearby stars will soon become the bottleneck for characterizing the atmospheres of small exoplanets via transmission spectroscopy. Using a carefully curated target list and more than two years' worth of APF-Levy and Keck-HIRES Doppler monitoring, the TESS-Keck Survey is working toward alleviating this pressure. Here we present mass measurements for 11 transiting planets in eight systems that are particularly suited to atmospheric follow-up with JWST. We also report the discovery and confirmation of a temperate super-Jovian-mass planet on a moderately eccentric orbit. The sample of eight host stars, which includes one subgiant, spans early-K to late-F spectral types ($T_\mathrm{eff} =$ 5200--6200 K). We homogeneously derive planet parameters using a joint photometry and radial velocity modeling framework, discuss the planets' possible bulk compositions, and comment on their prospects for atmospheric characterization.

==> rvobsstats.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% HIP 8152. System I %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\sysIhiresjObsStartEnd}{2019-Aug-14/2022-Jul-25}
\newcommand{\sysIhiresjNRVs}{94\xspace}
\newcommand{\sysIhiresjNbinnedRVs}{94\xspace}
\newcommand{\sysIhiresjNBinNoBinRVs}{94 (94)}
\newcommand{\sysIhiresjMedRVSNR}{213}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% HD 42813. System II %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\sysIIhiresjObsStartEnd}{2019-Sep-17/2022-Feb-22}
\newcommand{\sysIIhiresjNRVs}{71\xspace}
\newcommand{\sysIIhiresjNbinnedRVs}{71\xspace}
\newcommand{\sysIIhiresjNBinNoBinRVs}{71 (71)}
\newcommand{\sysIIhiresjMedRVSNR}{219}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% HD 25463. System III %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\sysIIIapfObsStartEnd}{2019-Aug-02/2020-Nov-16}
\newcommand{\sysIIIapfNRVs}{152\xspace}
\newcommand{\sysIIIapfNbinnedRVs}{124\xspace}
\newcommand{\sysIIIapfNBinNoBinRVs}{124 (152)}
\newcommand{\sysIIIapfMedRVSNR}{108}
\newcommand{\sysIIIhiresjObsStartEnd}{2019-Aug-14/2022-Feb-22}
\newcommand{\sysIIIhiresjNRVs}{265\xspace}
\newcommand{\sysIIIhiresjNbinnedRVs}{97\xspace}
\newcommand{\sysIIIhiresjNBinNoBinRVs}{97 (265)}
\newcommand{\sysIIIhiresjMedRVSNR}{213}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% TOI-669. System IV %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\sysIVhiresjObsStartEnd}{2019-Nov-07/2021-Nov-24}
\newcommand{\sysIVhiresjNRVs}{62\xspace}
\newcommand{\sysIVhiresjNbinnedRVs}{61\xspace}
\newcommand{\sysIVhiresjNBinNoBinRVs}{61 (62)}
\newcommand{\sysIVhiresjMedRVSNR}{150}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% HD 135694. System V %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\sysVapfObsStartEnd}{2019-Oct-25/2023-Jan-31}
\newcommand{\sysVapfNRVs}{150\xspace}
\newcommand{\sysVapfNbinnedRVs}{117\xspace}
\newcommand{\sysVapfNBinNoBinRVs}{117 (150)}
\newcommand{\sysVapfMedRVSNR}{68}
\newcommand{\sysVhiresjObsStartEnd}{2020-Jan-04/2022-Jul-09}
\newcommand{\sysVhiresjNRVs}{80\xspace}
\newcommand{\sysVhiresjNbinnedRVs}{79\xspace}
\newcommand{\sysVhiresjNBinNoBinRVs}{79 (80)}
\newcommand{\sysVhiresjMedRVSNR}{214}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% HIP 9618. System VI %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\sysVIapfObsStartEnd}{2020-Feb-19/2022-Nov-28}
\newcommand{\sysVIapfNRVs}{206\xspace}
\newcommand{\sysVIapfNbinnedRVs}{127\xspace}
\newcommand{\sysVIapfNBinNoBinRVs}{127 (206)}
\newcommand{\sysVIapfMedRVSNR}{80}
\newcommand{\sysVIhiresjObsStartEnd}{2020-Jan-21/2022-Jul-25}
\newcommand{\sysVIhiresjNRVs}{61\xspace}
\newcommand{\sysVIhiresjNbinnedRVs}{61\xspace}
\newcommand{\sysVIhiresjNBinNoBinRVs}{61 (61)}
\newcommand{\sysVIhiresjMedRVSNR}{214}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% HD 6061. System VII %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\sysVIIapfObsStartEnd}{2020-Jan-03/2022-Nov-22}
\newcommand{\sysVIIapfNRVs}{69\xspace}
\newcommand{\sysVIIapfNbinnedRVs}{56\xspace}
\newcommand{\sysVIIapfNBinNoBinRVs}{56 (69)}
\newcommand{\sysVIIapfMedRVSNR}{69}
\newcommand{\sysVIIhiresjObsStartEnd}{2019-Dec-16/2021-Aug-30}
\newcommand{\sysVIIhiresjNRVs}{64\xspace}
\newcommand{\sysVIIhiresjNbinnedRVs}{64\xspace}
\newcommand{\sysVIIhiresjNBinNoBinRVs}{64 (64)}
\newcommand{\sysVIIhiresjMedRVSNR}{212}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% TOI-1736. System VIII %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\sysVIIIapfObsStartEnd}{2021-Feb-18/2023-Jan-28}
\newcommand{\sysVIIIapfNRVs}{282\xspace}
\newcommand{\sysVIIIapfNbinnedRVs}{257\xspace}
\newcommand{\sysVIIIapfNBinNoBinRVs}{257 (282)}
\newcommand{\sysVIIIapfMedRVSNR}{85}
\newcommand{\sysVIIIhiresjObsStartEnd}{2020-Aug-02/2022-Jan-19}
\newcommand{\sysVIIIhiresjNRVs}{79\xspace}
\newcommand{\sysVIIIhiresjNbinnedRVs}{77\xspace}
\newcommand{\sysVIIIhiresjNBinNoBinRVs}{77 (79)}
\newcommand{\sysVIIIhiresjMedRVSNR}{203}

==> systemproperties.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% HIP 8152. System I %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mstarI}{$0.91 \pm 0.06$\xspace}
\newcommand{\rstarI}{$0.95 \pm 0.04$\xspace}
% Rtol threshold exceeded for u_0, so the posterior might be skewed
\newcommand{\uOneI}{$0.46 \pm 0.37$\xspace}
% Rtol threshold exceeded for u_1, so the posterior might be skewed
\newcommand{\uTwoI}{$0.09 \pm 0.39$\xspace}
\newcommand{\teffI}{$5530 \pm 110$\xspace}
\newcommand{\fehI}{$-0.09 \pm 0.09$\xspace}
\newcommand{\ageI}{$8.2 \pm 3.1$\xspace}

\newcommand{\periodIb}{$10.75101 \pm 0.00006$\xspace}
% Rtol threshold exceeded for period_c, so the posterior might be skewed
\newcommand{\periodIc}{$19.6053 \pm 0.0003$\xspace}
% Rtol threshold exceeded for t0_BTJD_b, so the posterior might be skewed
\newcommand{\tcBTJDIb}{$1758.620 \pm 0.002$\xspace}
\newcommand{\tcBTJDIc}{$1751.195 \pm 0.005$\xspace}
\newcommand{\rorIb}{$0.025 \pm 0.001$\xspace}
\newcommand{\rorIc}{$0.024 \pm 0.001$\xspace}
% Rtol threshold exceeded for b_b, so the posterior might be skewed
\newcommand{\bIb}{$0.67 \pm 0.07$\xspace}
% Rtol threshold exceeded for b_c, so the posterior might be skewed
\newcommand{\bIc}{$0.35 \pm 0.19$\xspace}
% Upper limit for ecc_b represents 98% confidence.
\newcommand{\eccIb}{$< 0.14$\xspace}
% Upper limit for ecc_c represents 98% confidence.
\newcommand{\eccIc}{$< 0.28$\xspace}
% Rtol threshold exceeded for omega_folded_deg_b, so the posterior might be skewed
\newcommand{\omegafoldeddegIb}{$161.8 \pm 137.1$\xspace}
% Rtol threshold exceeded for omega_folded_deg_c, so the posterior might be skewed
\newcommand{\omegafoldeddegIc}{$153.1 \pm 83.2$\xspace}
\newcommand{\KIb}{$2.42 \pm 0.53$\xspace}
\newcommand{\KIc}{$2.40 \pm 0.55$\xspace}
\newcommand{\aorIb}{$20.9 \pm 1.0$\xspace}
\newcommand{\aorIc}{$31.2 \pm 1.5$\xspace}
\newcommand{\aIb}{$0.092 \pm 0.002$\xspace}
\newcommand{\aIc}{$0.138 \pm 0.003$\xspace}
\newcommand{\rpIb}{$2.56 \pm 0.19$\xspace}
% Rtol threshold exceeded for rp_c, so the posterior might be skewed
\newcommand{\rpIc}{$2.48 \pm 0.19$\xspace}
\newcommand{\mpIb}{$7.8 \pm 1.8$\xspace}
\newcommand{\mpIc}{$9.4 \pm 2.2$\xspace}
% Rtol threshold exceeded for rho_b, so the posterior might be skewed
\newcommand{\rhoIb}{$2.5 \pm 0.8$\xspace}
% Rtol threshold exceeded for rho_c, so the posterior might be skewed
\newcommand{\rhoIc}{$3.4 \pm 1.1$\xspace}
\newcommand{\teqIb}{$855 \pm 28$\xspace}
\newcommand{\teqIc}{$699 \pm 23$\xspace}
% Rtol threshold exceeded for sinc_b, so the posterior might be skewed
\newcommand{\sincIb}{$88.9 \pm 11.6$\xspace}
% Rtol threshold exceeded for sinc_c, so the posterior might be skewed
\newcommand{\sincIc}{$39.9 \pm 5.2$\xspace}
% Rtol threshold exceeded for dur_hr_b, so the posterior might be skewed
\newcommand{\durhrIb}{$2.9 \pm 0.1$\xspace}
% Rtol threshold exceeded for dur_hr_c, so the posterior might be skewed
\newcommand{\durhrIc}{$4.3 \pm 0.3$\xspace}
% Rtol threshold exceeded for tsm_b, so the posterior might be skewed
\newcommand{\tsmIb}{$44 \pm 14$\xspace}
% Rtol threshold exceeded for tsm_c, so the posterior might be skewed
\newcommand{\tsmIc}{$27 \pm 9$\xspace}
% Rtol threshold exceeded for inc_b, so the posterior might be skewed
\newcommand{\inclIb}{$88.2 \pm 0.2$\xspace}
% Rtol threshold exceeded for inc_c, so the posterior might be skewed
\newcommand{\inclIc}{$89.3 \pm 0.4$\xspace}

\newcommand{\meanfluxI}{$0.009 \pm 0.006$\xspace}
% Rtol threshold exceeded for sigma_phot, so the posterior might be skewed
\newcommand{\sigmaphotI}{$0.01 \pm 0.01$\xspace}
\newcommand{\gammarvHIRESI}{$-1.44 \pm 0.37$\xspace}
% Rtol threshold exceeded for sigma_rv_HIRES, so the posterior might be skewed
\newcommand{\sigmarvHIRESI}{$3.15 \pm 0.30$\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% HD 42813. System II %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mstarII}{$0.94 \pm 0.06$\xspace}
% Rtol threshold exceeded for rstar, so the posterior might be skewed
\newcommand{\rstarII}{$0.97 \pm 0.03$\xspace}
\newcommand{\uOneII}{$0.37 \pm 0.23$\xspace}
% Rtol threshold exceeded for u_1, so the posterior might be skewed
\newcommand{\uTwoII}{$0.18 \pm 0.36$\xspace}
\newcommand{\teffII}{$5240 \pm 110$\xspace}
\newcommand{\fehII}{$0.33 \pm 0.09$\xspace}
\newcommand{\ageII}{$9.1 \pm 3.5$\xspace}

\newcommand{\periodIIb}{$13.63083 \pm 0.00003$\xspace}
\newcommand{\tcBTJDIIb}{$1842.6015 \pm 0.0007$\xspace}
\newcommand{\rorIIb}{$0.0317 \pm 0.0006$\xspace}
\newcommand{\bIIb}{$0.22 \pm 0.15$\xspace}
\newcommand{\eccIIb}{$\equiv 0$\xspace}
\newcommand{\omegafoldeddegIIb}{\nodata\xspace}
\newcommand{\KIIb}{$1.62 \pm 0.67$\xspace}
% Rtol threshold exceeded for aor_b, so the posterior might be skewed
\newcommand{\aorIIb}{$24.3 \pm 0.8$\xspace}
\newcommand{\aIIb}{$0.109 \pm 0.002$\xspace}
% Rtol threshold exceeded for rp_b, so the posterior might be skewed
\newcommand{\rpIIb}{$3.36 \pm 0.14$\xspace}
\newcommand{\mpIIb}{$5.8 \pm 2.4$\xspace}
\newcommand{\rhoIIb}{$0.8 \pm 0.4$\xspace}
% Rtol threshold exceeded for teq_b, so the posterior might be skewed
\newcommand{\teqIIb}{$755 \pm 21$\xspace}
% Rtol threshold exceeded for sinc_b, so the posterior might be skewed
\newcommand{\sincIIb}{$54.1 \pm 5.9$\xspace}
% Rtol threshold exceeded for dur_hr_b, so the posterior might be skewed
\newcommand{\durhrIIb}{$4.18 \pm 0.05$\xspace}
% Lower limit for tsm_b represents 98% confidence.
\newcommand{\tsmIIb}{$> 89$\xspace}
\newcommand{\inclIIb}{$89.5 \pm 0.4$\xspace}

\newcommand{\meanfluxII}{$0.02 \pm 0.03$\xspace}
\newcommand{\sigmaphotII}{$0.170 \pm 0.008$\xspace}
\newcommand{\gammarvHIRESII}{$-0.39 \pm 0.42$\xspace}
% Rtol threshold exceeded for sigma_rv_HIRES, so the posterior might be skewed
\newcommand{\sigmarvHIRESII}{$3.21 \pm 0.32$\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% HD 25463. System III %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mstarIII}{$1.19 \pm 0.07$\xspace}
\newcommand{\rstarIII}{$1.41 \pm 0.07$\xspace}
% Rtol threshold exceeded for u_0, so the posterior might be skewed
\newcommand{\uOneIII}{$0.42 \pm 0.31$\xspace}
\newcommand{\uTwoIII}{$0.05 \pm 0.33$\xspace}
\newcommand{\teffIII}{$6220 \pm 110$\xspace}
\newcommand{\fehIII}{$-0.20 \pm 0.09$\xspace}
\newcommand{\ageIII}{$3.1 \pm 0.7$\xspace}

\newcommand{\periodIIIb}{$7.049144 \pm 0.000009$\xspace}
% Rtol threshold exceeded for period_c, so the posterior might be skewed
\newcommand{\periodIIIc}{$3.044050 \pm 0.000008$\xspace}
\newcommand{\tcBTJDIIIb}{$1978.3531 \pm 0.0006$\xspace}
\newcommand{\tcBTJDIIIc}{$1980.314 \pm 0.001$\xspace}
% Rtol threshold exceeded for ror_b, so the posterior might be skewed
\newcommand{\rorIIIb}{$0.0170 \pm 0.0004$\xspace}
\newcommand{\rorIIIc}{$0.0098 \pm 0.0006$\xspace}
% Rtol threshold exceeded for b_b, so the posterior might be skewed
\newcommand{\bIIIb}{$0.72 \pm 0.04$\xspace}
\newcommand{\bIIIc}{$0.93 \pm 0.01$\xspace}
\newcommand{\eccIIIb}{$\equiv 0$\xspace}
\newcommand{\eccIIIc}{$\equiv 0$\xspace}
\newcommand{\omegafoldeddegIIIb}{\nodata\xspace}
\newcommand{\omegafoldeddegIIIc}{\nodata\xspace}
\newcommand{\KIIIb}{$2.54 \pm 0.90$\xspace}
% Upper limit for K_c represents 98% confidence.
\newcommand{\KIIIc}{$< 1.60$\xspace}
% Rtol threshold exceeded for aor_b, so the posterior might be skewed
\newcommand{\aorIIIb}{$11.6 \pm 0.6$\xspace}
% Rtol threshold exceeded for aor_c, so the posterior might be skewed
\newcommand{\aorIIIc}{$6.6 \pm 0.3$\xspace}
\newcommand{\aIIIb}{$0.076 \pm 0.002$\xspace}
\newcommand{\aIIIc}{$0.0435 \pm 0.0009$\xspace}
\newcommand{\rpIIIb}{$2.62 \pm 0.16$\xspace}
\newcommand{\rpIIIc}{$1.50 \pm 0.12$\xspace}
\newcommand{\mpIIIb}{$8.5 \pm 3.1$\xspace}
% Upper limit for mp_c represents 98% confidence.
\newcommand{\mpIIIc}{$< 4.1$\xspace}
% Rtol threshold exceeded for rho_b, so the posterior might be skewed
\newcommand{\rhoIIIb}{$2.6 \pm 1.1$\xspace}
% Upper limit for rho_c represents 98% confidence.
\newcommand{\rhoIIIc}{$< 7.1$\xspace}
\newcommand{\teqIIIb}{$1290 \pm 41$\xspace}
\newcommand{\teqIIIc}{$1707 \pm 54$\xspace}
% Rtol threshold exceeded for sinc_b, so the posterior might be skewed
\newcommand{\sincIIIb}{$461.4 \pm 58.7$\xspace}
% Rtol threshold exceeded for sinc_c, so the posterior might be skewed
\newcommand{\sincIIIc}{$1413.5 \pm 179.7$\xspace}
\newcommand{\durhrIIIb}{$3.23 \pm 0.04$\xspace}
\newcommand{\durhrIIIc}{$1.30 \pm 0.05$\xspace}
% Rtol threshold exceeded for tsm_b, so the posterior might be skewed
\newcommand{\tsmIIIb}{$112 \pm 51$\xspace}
% Lower limit for tsm_c represents 98% confidence.
\newcommand{\tsmIIIc}{$> 55$\xspace}
\newcommand{\inclIIIb}{$86.4 \pm 0.4$\xspace}
\newcommand{\inclIIIc}{$81.9 \pm 0.5$\xspace}

\newcommand{\meanfluxIII}{$0.006 \pm 0.005$\xspace}
\newcommand{\sigmaphotIII}{$0.122 \pm 0.001$\xspace}
\newcommand{\gammarvAPFIII}{$0.33 \pm 0.88$\xspace}
\newcommand{\sigmarvAPFIII}{$7.34 \pm 0.80$\xspace}
\newcommand{\gammarvHIRESIII}{$-1.97 \pm 0.80$\xspace}
% Rtol threshold exceeded for sigma_rv_HIRES, so the posterior might be skewed
\newcommand{\sigmarvHIRESIII}{$7.31 \pm 0.61$\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% TOI-669. System IV %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mstarIV}{$0.90 \pm 0.06$\xspace}
\newcommand{\rstarIV}{$0.99 \pm 0.04$\xspace}
\newcommand{\uOneIV}{$0.88 \pm 0.43$\xspace}
% Rtol threshold exceeded for u_1, so the posterior might be skewed
\newcommand{\uTwoIV}{$-0.18 \pm 0.41$\xspace}
\newcommand{\teffIV}{$5600 \pm 110$\xspace}
\newcommand{\fehIV}{$-0.06 \pm 0.09$\xspace}
\newcommand{\ageIV}{$8.6 \pm 2.9$\xspace}

\newcommand{\periodIVb}{$3.94515 \pm 0.00002$\xspace}
\newcommand{\tcBTJDIVb}{$1913.041 \pm 0.002$\xspace}
\newcommand{\rorIVb}{$0.024 \pm 0.001$\xspace}
% Rtol threshold exceeded for b_b, so the posterior might be skewed
\newcommand{\bIVb}{$0.23 \pm 0.18$\xspace}
% Upper limit for ecc_b represents 98% confidence.
\newcommand{\eccIVb}{$< 0.23$\xspace}
\newcommand{\omegafoldeddegIVb}{$196.2 \pm 64.3$\xspace}
\newcommand{\KIVb}{$4.30 \pm 0.62$\xspace}
\newcommand{\aorIVb}{$10.3 \pm 0.5$\xspace}
\newcommand{\aIVb}{$0.047 \pm 0.001$\xspace}
% Rtol threshold exceeded for rp_b, so the posterior might be skewed
\newcommand{\rpIVb}{$2.60 \pm 0.17$\xspace}
\newcommand{\mpIVb}{$9.8 \pm 1.5$\xspace}
% Rtol threshold exceeded for rho_b, so the posterior might be skewed
\newcommand{\rhoIVb}{$3.0 \pm 0.7$\xspace}
\newcommand{\teqIVb}{$1235 \pm 37$\xspace}
% Rtol threshold exceeded for sinc_b, so the posterior might be skewed
\newcommand{\sincIVb}{$388.2 \pm 47.1$\xspace}
% Rtol threshold exceeded for dur_hr_b, so the posterior might be skewed
\newcommand{\durhrIVb}{$2.9 \pm 0.1$\xspace}
% Rtol threshold exceeded for tsm_b, so the posterior might be skewed
\newcommand{\tsmIVb}{$35 \pm 8$\xspace}
\newcommand{\inclIVb}{$88.7 \pm 1.0\degree$\xspace}

\newcommand{\meanfluxIV}{$0.02 \pm 0.01$\xspace}
% Rtol threshold exceeded for sigma_phot, so the posterior might be skewed
\newcommand{\sigmaphotIV}{$0.02 \pm 0.02$\xspace}
\newcommand{\gammarvHIRESIV}{$-2.25 \pm 0.43$\xspace}
% Rtol threshold exceeded for sigma_rv_HIRES, so the posterior might be skewed
\newcommand{\sigmarvHIRESIV}{$2.88 \pm 0.36$\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% HD 135694. System V %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mstarV}{$0.90 \pm 0.06$\xspace}
\newcommand{\rstarV}{$1.05 \pm 0.05$\xspace}
% Rtol threshold exceeded for u_0, so the posterior might be skewed
\newcommand{\uOneV}{$0.15 \pm 0.16$\xspace}
% Rtol threshold exceeded for u_1, so the posterior might be skewed
\newcommand{\uTwoV}{$0.51 \pm 0.28$\xspace}
\newcommand{\teffV}{$5710 \pm 110$\xspace}
\newcommand{\fehV}{$-0.21 \pm 0.09$\xspace}
\newcommand{\ageV}{$9.6 \pm 2.4$\xspace}

% Rtol threshold exceeded for period_b, so the posterior might be skewed
\newcommand{\periodVb}{$15.92346 \pm 0.00002$\xspace}
\newcommand{\tcBTJDVb}{$2324.5878 \pm 0.0007$\xspace}
% Rtol threshold exceeded for ror_b, so the posterior might be skewed
\newcommand{\rorVb}{$0.0219 \pm 0.0005$\xspace}
\newcommand{\bVb}{$0.37 \pm 0.23$\xspace}
% Upper limit for ecc_b represents 98% confidence.
\newcommand{\eccVb}{$< 0.42$\xspace}
% Rtol threshold exceeded for omega_folded_deg_b, so the posterior might be skewed
\newcommand{\omegafoldeddegVb}{$82.5 \pm 152.4$\xspace}
\newcommand{\KVb}{$1.60 \pm 0.58$\xspace}
% Rtol threshold exceeded for aor_b, so the posterior might be skewed
\newcommand{\aorVb}{$24.5 \pm 1.3$\xspace}
\newcommand{\aVb}{$0.120 \pm 0.003$\xspace}
\newcommand{\rpVb}{$2.51 \pm 0.14$\xspace}
\newcommand{\mpVb}{$5.7 \pm 2.1$\xspace}
% Rtol threshold exceeded for rho_b, so the posterior might be skewed
\newcommand{\rhoVb}{$2.0 \pm 0.8$\xspace}
\newcommand{\teqVb}{$815 \pm 27$\xspace}
% Rtol threshold exceeded for sinc_b, so the posterior might be skewed
\newcommand{\sincVb}{$73.7 \pm 9.9$\xspace}
% Rtol threshold exceeded for dur_hr_b, so the posterior might be skewed
\newcommand{\durhrVb}{$4.29 \pm 0.05$\xspace}
% Rtol threshold exceeded for tsm_b, so the posterior might be skewed
\newcommand{\tsmVb}{$69 \pm 32$\xspace}
% Rtol threshold exceeded for inc_b, so the posterior might be skewed
\newcommand{\inclVb}{$89.1 \pm 0.5\degree$\xspace}

\newcommand{\meanfluxV}{$0.012 \pm 0.004$\xspace}
\newcommand{\sigmaphotV}{$0.074 \pm 0.005$\xspace}
\newcommand{\gammarvAPFV}{$0.50 \pm 0.71$\xspace}
% Rtol threshold exceeded for sigma_rv_APF, so the posterior might be skewed
\newcommand{\sigmarvAPFV}{$7.08 \pm 0.54$\xspace}
\newcommand{\gammarvHIRESV}{$0.03 \pm 0.47$\xspace}
% Rtol threshold exceeded for sigma_rv_HIRES, so the posterior might be skewed
\newcommand{\sigmarvHIRESV}{$3.78 \pm 0.36$\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% HIP 9618. System VI %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mstarVI}{$0.93 \pm 0.06$\xspace}
% Rtol threshold exceeded for rstar, so the posterior might be skewed
\newcommand{\rstarVI}{$0.95 \pm 0.03$\xspace}
\newcommand{\uOneVI}{$0.37 \pm 0.19$\xspace}
% Rtol threshold exceeded for u_1, so the posterior might be skewed
\newcommand{\uTwoVI}{$0.17 \pm 0.31$\xspace}
\newcommand{\teffVI}{$5550 \pm 110$\xspace}
\newcommand{\fehVI}{$-0.1 \pm 0.09$\xspace}
\newcommand{\ageVI}{$5.2 \pm 2.7$\xspace}

\newcommand{\periodVIb}{$20.77288 \pm 0.00005$\xspace}
\newcommand{\periodVIc}{$52.5636 \pm 0.0002$\xspace}
\newcommand{\tcBTJDVIb}{$2120.5612 \pm 0.0008$\xspace}
\newcommand{\tcBTJDVIc}{$2094.572 \pm 0.001$\xspace}
\newcommand{\rorVIb}{$0.0364 \pm 0.0005$\xspace}
\newcommand{\rorVIc}{$0.0324 \pm 0.0006$\xspace}
% Rtol threshold exceeded for b_b, so the posterior might be skewed
\newcommand{\bVIb}{$0.17 \pm 0.13$\xspace}
\newcommand{\bVIc}{$0.24 \pm 0.14$\xspace}
% Upper limit for ecc_b represents 98% confidence.
\newcommand{\eccVIb}{$< 0.13$\xspace}
% Upper limit for ecc_c represents 98% confidence.
\newcommand{\eccVIc}{$< 0.12$\xspace}
% Rtol threshold exceeded for omega_folded_deg_b, so the posterior might be skewed
\newcommand{\omegafoldeddegVIb}{$206.6 \pm 147.8$\xspace}
% Rtol threshold exceeded for omega_folded_deg_c, so the posterior might be skewed
\newcommand{\omegafoldeddegVIc}{$165.6 \pm 130.8$\xspace}
\newcommand{\KVIb}{$2.06 \pm 0.48$\xspace}
% Upper limit for K_c represents 98% confidence.
\newcommand{\KVIc}{$< 1.41$\xspace}
% Rtol threshold exceeded for aor_b, so the posterior might be skewed
\newcommand{\aorVIb}{$32.9 \pm 0.9$\xspace}
% Rtol threshold exceeded for aor_c, so the posterior might be skewed
\newcommand{\aorVIc}{$61.0 \pm 1.7$\xspace}
\newcommand{\aVIb}{$0.144 \pm 0.003$\xspace}
\newcommand{\aVIc}{$0.268 \pm 0.006$\xspace}
% Rtol threshold exceeded for rp_b, so the posterior might be skewed
\newcommand{\rpVIb}{$3.75 \pm 0.13$\xspace}
% Rtol threshold exceeded for rp_c, so the posterior might be skewed
\newcommand{\rpVIc}{$3.34 \pm 0.13$\xspace}
\newcommand{\mpVIb}{$8.4 \pm 2.0$\xspace}
% Upper limit for mp_c represents 98% confidence.
\newcommand{\mpVIc}{$< 7.9$\xspace}
\newcommand{\rhoVIb}{$0.9 \pm 0.2$\xspace}
% Upper limit for rho_c represents 98% confidence.
\newcommand{\rhoVIc}{$< 1.2$\xspace}
\newcommand{\teqVIb}{$685 \pm 17$\xspace}
\newcommand{\teqVIc}{$503 \pm 13$\xspace}
% Rtol threshold exceeded for sinc_b, so the posterior might be skewed
\newcommand{\sincVIb}{$36.8 \pm 3.7$\xspace}
% Rtol threshold exceeded for sinc_c, so the posterior might be skewed
\newcommand{\sincVIc}{$10.7 \pm 1.1$\xspace}
% Rtol threshold exceeded for dur_hr_b, so the posterior might be skewed
\newcommand{\durhrVIb}{$4.74 \pm 0.05$\xspace}
% Rtol threshold exceeded for dur_hr_c, so the posterior might be skewed
\newcommand{\durhrVIc}{$6.34 \pm 0.06$\xspace}
% Rtol threshold exceeded for tsm_b, so the posterior might be skewed
\newcommand{\tsmVIb}{$161 \pm 43$\xspace}
% Lower limit for tsm_c represents 98% confidence.
\newcommand{\tsmVIc}{$> 87$\xspace}
\newcommand{\inclVIb}{$89.7 \pm 0.2$\xspace}
% Rtol threshold exceeded for inc_c, so the posterior might be skewed
\newcommand{\inclVIc}{$89.8 \pm 0.1$\xspace}

\newcommand{\trendrvslopeVI}{$-0.059 \pm 0.001$\xspace}
% Rtol threshold exceeded for mean_flux, so the posterior might be skewed
\newcommand{\meanfluxVI}{$0.022 \pm 0.009$\xspace}
\newcommand{\sigmaphotVI}{$0.148 \pm 0.006$\xspace}
\newcommand{\gammarvAPFVI}{$11.34 \pm 0.52$\xspace}
% Rtol threshold exceeded for sigma_rv_APF, so the posterior might be skewed
\newcommand{\sigmarvAPFVI}{$4.81 \pm 0.38$\xspace}
\newcommand{\gammarvHIRESVI}{$0.57 \pm 0.48$\xspace}
% Rtol threshold exceeded for sigma_rv_HIRES, so the posterior might be skewed
\newcommand{\sigmarvHIRESVI}{$3.34 \pm 0.42$\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% HD 6061. System VII %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mstarVII}{$1.00 \pm 0.06$\xspace}
% Rtol threshold exceeded for rstar, so the posterior might be skewed
\newcommand{\rstarVII}{$1.03 \pm 0.03$\xspace}
% Rtol threshold exceeded for u_0, so the posterior might be skewed
\newcommand{\uOneVII}{$0.28 \pm 0.24$\xspace}
\newcommand{\uTwoVII}{$0.35 \pm 0.36$\xspace}
\newcommand{\teffVII}{$5920 \pm 110$\xspace}
\newcommand{\fehVII}{$-0.08 \pm 0.09$\xspace}
\newcommand{\ageVII}{$2.4 \pm 1.7$\xspace}

\newcommand{\periodVIIb}{$5.254467 \pm 0.000009$\xspace}
\newcommand{\tcBTJDVIIb}{$2321.505 \pm 0.001$\xspace}
\newcommand{\rorVIIb}{$0.0218 \pm 0.0006$\xspace}
% Rtol threshold exceeded for b_b, so the posterior might be skewed
\newcommand{\bVIIb}{$0.14 \pm 0.12$\xspace}
\newcommand{\eccVIIb}{$\equiv 0$\xspace}
\newcommand{\omegafoldeddegVIIb}{\nodata\xspace}
\newcommand{\KVIIb}{$4.00 \pm 0.99$\xspace}
\newcommand{\aorVIIb}{$12.3 \pm 0.3$\xspace}
\newcommand{\aVIIb}{$0.059 \pm 0.001$\xspace}
% Rtol threshold exceeded for rp_b, so the posterior might be skewed
\newcommand{\rpVIIb}{$2.45 \pm 0.09$\xspace}
\newcommand{\mpVIIb}{$10.8 \pm 2.7$\xspace}
\newcommand{\rhoVIIb}{$4.0 \pm 1.1$\xspace}
\newcommand{\teqVIIb}{$1194 \pm 28$\xspace}
% Rtol threshold exceeded for sinc_b, so the posterior might be skewed
\newcommand{\sincVIIb}{$339.1 \pm 31.9$\xspace}
% Rtol threshold exceeded for dur_hr_b, so the posterior might be skewed
\newcommand{\durhrVIIb}{$3.21 \pm 0.06$\xspace}
% Rtol threshold exceeded for tsm_b, so the posterior might be skewed
\newcommand{\tsmVIIb}{$55 \pm 16$\xspace}
% Rtol threshold exceeded for inc_b, so the posterior might be skewed
\newcommand{\inclVIIb}{$89.3 \pm 0.6$\xspace}

\newcommand{\meanfluxVII}{$0.03 \pm 0.05$\xspace}
\newcommand{\sigmaphotVII}{$0.150 \pm 0.005$\xspace}
\newcommand{\gammarvAPFVII}{$0.58 \pm 1.79$\xspace}
% Rtol threshold exceeded for sigma_rv_APF, so the posterior might be skewed
\newcommand{\sigmarvAPFVII}{$2.80 \pm 3.96$\xspace}
\newcommand{\gammarvHIRESVII}{$-2.57 \pm 1.02$\xspace}
% Rtol threshold exceeded for sigma_rv_HIRES, so the posterior might be skewed
\newcommand{\sigmarvHIRESVII}{$2.17 \pm 2.01$\xspace}
\newcommand{\gpsvaluemeanVII}{$0.205 \pm 0.002$\xspace}
% Rtol threshold exceeded for sigma_svalue, so the posterior might be skewed
\newcommand{\sigmasvalueVII}{$0.0003 \pm 0.0004$\xspace}
\newcommand{\protrvsvaluegpVII}{$13.9 \pm 1.6$\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% TOI-1736. System VIII %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mstarVIII}{$1.06 \pm 0.08$\xspace}
\newcommand{\rstarVIII}{$1.38 \pm 0.07$\xspace}
% Rtol threshold exceeded for u_0, so the posterior might be skewed
\newcommand{\uOneVIII}{$0.19 \pm 0.19$\xspace}
\newcommand{\uTwoVIII}{$0.26 \pm 0.27$\xspace}
\newcommand{\teffVIII}{$5670 \pm 110$\xspace}
\newcommand{\fehVIII}{$0.13 \pm 0.09$\xspace}
\newcommand{\ageVIII}{$8.6 \pm 1.7$\xspace}

\newcommand{\periodVIIIb}{$7.073091 \pm 0.000008$\xspace}
\newcommand{\tcBTJDVIIIb}{$2740.5891 \pm 0.0007$\xspace}
\newcommand{\rorVIIIb}{$0.0202 \pm 0.0004$\xspace}
% Rtol threshold exceeded for b_b, so the posterior might be skewed
\newcommand{\bVIIIb}{$0.53 \pm 0.11$\xspace}
% Upper limit for ecc_b represents 98% confidence.
\newcommand{\eccVIIIb}{$< 0.16$\xspace}
% Rtol threshold exceeded for omega_folded_deg_b, so the posterior might be skewed
\newcommand{\omegafoldeddegVIIIb}{$136.4 \pm 94.5$\xspace}
\newcommand{\KVIIIb}{$3.82 \pm 0.49$\xspace}
% Rtol threshold exceeded for aor_b, so the posterior might be skewed
\newcommand{\aorVIIIb}{$11.4 \pm 0.6$\xspace}
\newcommand{\aVIIIb}{$0.074 \pm 0.002$\xspace}
\newcommand{\rpVIIIb}{$3.05 \pm 0.19$\xspace}
\newcommand{\mpVIIIb}{$11.9 \pm 1.6$\xspace}
% Rtol threshold exceeded for rho_b, so the posterior might be skewed
\newcommand{\rhoVIIIb}{$2.3 \pm 0.5$\xspace}
\newcommand{\teqVIIIb}{$1186 \pm 41$\xspace}
% Rtol threshold exceeded for sinc_b, so the posterior might be skewed
\newcommand{\sincVIIIb}{$329.6 \pm 46.0$\xspace}
% Rtol threshold exceeded for dur_hr_b, so the posterior might be skewed
\newcommand{\durhrVIIIb}{$3.94 \pm 0.04$\xspace}
% Rtol threshold exceeded for tsm_b, so the posterior might be skewed
\newcommand{\tsmVIIIb}{$55 \pm 11$\xspace}
% Rtol threshold exceeded for inc_b, so the posterior might be skewed
\newcommand{\inclVIIIb}{$87.3 \pm 0.7$\xspace}
\newcommand{\msiniVIIIb}{$11.9 \pm 1.6$\xspace}
\newcommand{\msinijupVIIIb}{$0.037 \pm 0.005$\xspace}
\newcommand{\nontransperiodVIIIc}{$571.3 \pm 0.5$\xspace}
\newcommand{\nontranstcBTJDVIIIc}{$2273.1 \pm 0.4$\xspace}
\newcommand{\nontranseccVIIIc}{$0.369 \pm 0.002$\xspace}
\newcommand{\nontransomegafoldeddegVIIIc}{$162.1 \pm 0.5$\xspace}
\newcommand{\nontransKVIIIc}{$197.6 \pm 0.6$\xspace}
% Rtol threshold exceeded for nontrans_aor_c, so the posterior might be skewed
\newcommand{\nontransaorVIIIc}{$213.4 \pm 12.1$\xspace}
\newcommand{\nontransaVIIIc}{$1.37 \pm 0.03$\xspace}
\newcommand{\nontransmsiniVIIIc}{$2477 \pm 118$\xspace}
\newcommand{\nontransteqVIIIc}{$274 \pm 10$\xspace}
% Rtol threshold exceeded for nontrans_sinc_c, so the posterior might be skewed
\newcommand{\nontranssincVIIIc}{$0.9 \pm 0.1$\xspace}
\newcommand{\nontransmsinijupVIIIc}{$7.8 \pm 0.4$\xspace}

\newcommand{\trendrvslopeVIII}{$-0.183 \pm 0.002$\xspace}
\newcommand{\meanfluxVIII}{$0.012 \pm 0.006$\xspace}
\newcommand{\sigmaphotVIII}{$0.117 \pm 0.004$\xspace}
\newcommand{\gammarvAPFVIII}{$23.59 \pm 0.80$\xspace}
\newcommand{\sigmarvAPFVIII}{$6.15 \pm 0.32$\xspace}
\newcommand{\gammarvHIRESVIII}{$19.99 \pm 0.59$\xspace}
% Rtol threshold exceeded for sigma_rv_HIRES, so the posterior might be skewed
\newcommand{\sigmarvHIRESVIII}{$4.34 \pm 0.45$\xspace}
